Computing m-Eternal Domination Number of Cactus Graphs in Linear Time

In m-eternal domination attacker and defender play on a graph. Initially, the defender places guards on vertices. In each round, the attacker chooses a vertex to attack. Then, the defender can move each guard to a neighboring vertex and must move a guard to the attacked vertex. The m-eternal domination number is the minimum number of guards such that the graph can be defended indefinitely. In this paper, we study the m-eternal domination number of cactus graphs. We consider two variants of the m-eternal domination number: one allows multiple guards to occupy a single vertex, the second variant requires the guards to occupy distinct vertices. We develop several tools for obtaining lower and upper bounds on these problems and we use them to obtain an algorithm which computes the minimum number of required guards of cactus graphs for both variants of the problem.

==> cactus.tex <==
\section{Linear algorithm for m-eternal domination number of cactus graphs}

We will say that a vertex is \textit{red} if it is incident to at least two leaves. Also any vertex incident to at least one leaf and at least one red vertex is also red.

We will say that an edge is \textit{green} if there exists a strategy, such that there are no two neighboring configurations in which there is a movement along the edge in the same direction. Also it can not hold that both endpoints are red.


Each of the following reductions will inductively show the following.
In at least one optimal m-eternal domination strategy, it holds that
\begin{itemize}
  \item Every attack can be defended
  \item Every non-red vertex can be evicted.
  \item Every edge with no red endpoints, which is also on a cycle, can be evicted.
  \item Every cycle edge with at most one red vertex is green. (Property 2)
  \item Every red vertex is always occupied in some optimal strategy
  \item There is an optimal strategy such that we can forbid one directed movement starting in a red vertex for this and the next turn and the strategy is still valid (all of the previous holds). We can therefore perform an attack/eviction and then ask that a movement is not used in the next turn.
  \item Instead of an attack or eviction, we can request that a movement happens over some red-free edge in which exactly one endpoint is occupied.
\end{itemize}
Moreover, every reduction has known its exact change in optimal number of guards.

The base case consists of a single vertex, single edge and a simple cycle. All of the mentioned properties hold, and the minimum required number of guards is easy to compute.



\begin{lemma}\label{lem:red-vertices}
  There exists an m-eternal guard strategy of $G$ such that every red vertex is always occupied.
\end{lemma}
\begin{proof}
  Let $r_1, r_2, \dots, r_k$ be the set of all red vertices in $G$.
  Let $l_i = \{l_{i,1}, l_{i,2}, \dots l_{i,k_i}\}$ be the leaves attached to $r_i$.
  Suppose $S_G$ contains the lowest possible number of $C$ such that some $r_i$ is not occupied.
  By Lemma \ref{lem:strategy-transform} we can get a strategy $S'_G$ where at most one of vertices in $l_i$ is occupied at any time.
  Let $l_{i,j}$ be the unoccupied vertex. For it to be defended, there must be a guard at $r_i$ as it is its only neighbor.
\end{proof}











\begin{figure}[h]\centering
  \includegraphics[width=75pt]{images/cactus-reductions/star2.png}
  \caption[Reduction~\ref{rdc:star2}]{%
    }%
    \label{fig:star2}
    Reduction \ref{rdc:star2}
\end{figure}

\begin{restatable}{reduction}{reduction-star2}
  \label{rdc:star2}
  Contract the edge connecting the red vertices
\end{restatable}
\begin{lemma}
  Reduction \ref{rdc:star2} is correct.
\end{lemma}
\begin{proof}

  \lowerbound

  Follows from Lemma~\ref{lem:contract-occupied-edge}

  \upperbound

  Let $r_2$ be the removed red vertex, $r_1$ is the one left. Any movement of a guard outside of $r_1$ and into $r_1$ can be performed along $r_2$ as well.

  \begin{itemize}
    \item The the leaves can still be defended
    \item The leaf vertices can still be evicted.
    \item No edge without red enpoints is created.
    \item No edge with no red vertices is green. (Property 2)
  \end{itemize}

\end{proof}








\begin{figure}[h]\centering
  \includegraphics[width=350pt]{images/cactus-reductions/star3.png}
  \caption[Reduction~\ref{rdc:star3}]{%
    }%
    \label{fig:star3}
    Reduction \ref{rdc:star3}
\end{figure}

\begin{restatable}{reduction}{reduction-star3}
  \label{rdc:star3}
  Contract into an edge as in the image and remove 3 guards.
\end{restatable}
\begin{lemma}
  Reduction \ref{rdc:star3} is correct.
\end{lemma}
\begin{proof}

  \lowerbound

  Follows from the sequence of reductions using Lemma \ref{lem:contract-subgraph}

  \upperbound

28 - 001110000: 28 29 31 54 86 151 279 

29 - 101110000: 28 29 31 54 86 151 279 

31 - 111110000: 28 29 31 54 86 151 279 

54 - 011011000: 28 29 31 54 86 151 279 

86 - 011010100: 28 29 31 54 86 151 279 

151 - 111010010: 28 29 31 54 86 151 279 

279 - 111010001: 28 29 31 54 86 151 279 

  \begin{itemize}
    \item Shows the table
    \item Shows the table
    \item No edge without red enpoints is created.
    \item No green edge is present.
  \end{itemize}

\end{proof}












\begin{figure}[h]\centering
  \includegraphics[width=75pt]{images/cactus-reductions/star1.png}
  \caption[Reduction~\ref{rdc:star1}]{%
    Reduction \ref{rdc:star1}.
    Red vertices: 4.
    }%
    \label{fig:bull-lowerbound}
\end{figure}

\begin{restatable}{reduction}{reduction-star1}
  \label{rdc:star1}
  Contract the subgraph $S$ into vertex $0$ and remove 2 guards.
\end{restatable}

\begin{lemma}
  Reduction \ref{rdc:star1} is correct.
\end{lemma}
\begin{proof}

  \lowerbound

  $s = (l_1, l_2)$

  \upperbound

  \begin{tabular}{|c|c|c|c|}
    \hline
    State & Neighborhood of $S$ & Vertices of $S$ (defends) & Evicts\\
    \hline
    $m_0$ & $\{1\}, \{0, 1\}$ & $\{\textbf{2}, \textbf{4}\}$ & $\{3, 5, 6\}$\\
    \hline
    $m_1$ & $\{0\}, \{0, 1\}$ & $\{\textbf{3}, 4\}$ & $\{2, 5, 6\}$\\
    \hline
    $d_1$ & $\emptyset$ & $\{4, \textbf{6}\}$ & $\{\textbf{2}, \textbf{3}, \textbf{5}\}$\\
    \hline
    $d_2$ & $\emptyset$ & $\{4, \textbf{5}\}$ & $\{2, 3, \textbf{6}\}$\\
    \hline
  \end{tabular}
  \begin{itemize}

    \item Changes of the neighborhood of $S$ not with moving over the $\{0,1\}$ edge.

      \begin{tabular}{|c|c|c|c|c|}
        \hline
         &     $\emptyset$ & $\{0\}$ & $\{1\}$ & $\{0, 1\}$\\
        \hline
        $\emptyset$ & $d_1$ & $m_1$ & $m_0$ & $m_0$ \\
        \hline
        $\{0\}, \{0, 1\}$ & $d_1$ & $m_1$ & $m_0$ & $m_0$ \\
        \hline
        $\{1\}, \{0, 1\}$ & $d_1$ & $m_1$ & $m_0$ & $m_0$ \\
        \hline
        $\{0, 1\}$ & $d_1$ & $m_1$ & $m_0$ & $m_0$ \\
        \hline
      \end{tabular}

    \item Changes of the neighborhood of $S$ with moving over the $\{0,1\}$ edge.

      \begin{tabular}{|c|c|c|c|c|}
        \hline
         & $\{0\}$ & $\{1\}$ & $\{0, 1\}$\\
        \hline
        $\{0\}$ & & $(m_1, m_0)$ & $(m_1, m_0)$  \\
        \hline
        $\{1\}$ & $(m_0, m_1)$ & & $(m_0, m_1)$ \\
        \hline
        $\{0, 1\}$ & does not happend on a green edge & & equivalent to no movement \\
        \hline
      \end{tabular}

\item Cycle edge eviction: $\{0,2\}$ and $\{1,3\}$ can be evicted by moving into $d_1$.

%\item Property 1: Clearly holds for edges with a leaf endpoint.
  %For $\{0,2\}$ or $\{1,3\}$ to be passed twice in a row in the same direction, the resulting $\{0,1\}$ edges would have to be passed twice.
      %But this does not happen by the induction hypothesis.

    \item Property 2: We will show that $\{0, 2\}$ and $\{1, 3\}$ are green. WLOG consider $\{0, 2\}$. Movement over over the edge
      happens only when movement happens over $\{0, 1\}$ in the reduced graph.
      Because $\{0, 1\}$ is green, the movement only happens when exactly one endpoint is occupied. Therefore the movement over $\{0, 2\}$ also happens only when $0$ is not occupied.

    \item Edges $\{2, 4\}$ can $\{3, 4\}$ can be forbidden for one turn. WLOG we want to forbid $\{2, 4\}$. The movement across this edge may happen to simulate movement over $(0,1)$ or defend $2$.

      First suppose that $2$ is occupied at the start of this request. Then we evict $\{0,1\}$ so the movement will not happen and defending $2$ is trivial.
      Otherwise one of $3,5,6$ are occupied.
      Then move the guard to $3$ and simulate an attack on $0$.
      To defend $2$ we then request the movement across $(1,0)$.
  \end{itemize}

%22 - 0110100: 22 25 80 83 99 
%25 - 1001100: 22 25 80 83 99 
%80 - 0000101: 22 25 80 83 99 
%83 - 1100101: 22 25 80 83 99 
%99 - 1100011: 22 25 80 83 99 

\end{proof}
















\begin{figure}[h]\centering
  \includegraphics[width=350pt]{images/cactus-reductions/p2.png}
  \caption[Reduction~\ref{rdc:p2}]{%
    }%
    Reduction \ref{rdc:p2}
    \label{fig:p2}
\end{figure}
\begin{restatable}{reduction}{reduction-p2}
  \label{rdc:p2}
  Contract the subgraph $P_2$ into $x$ and remove 1 guards.
\end{restatable}

\begin{lemma}
  Reduction \ref{rdc:p2} is correct.
\end{lemma}
\begin{proof}

  \lowerbound

  $s = (v_2)$

  \upperbound


%5 - 1010: 5 6 8 11 
%6 - 0110: 5 6 8 11 
%8 - 0001: 5 6 8 11 
%11 - 1101: 5 6 8 11 

6 - 01100: 6 8 11 17 

8 - 00010: 6 8 11 17 

11 - 11010: 6 8 11 17 

17 - 10001: 6 8 11 17 

  \begin{itemize}
    \item Shows the table
    \item Shows the table
    \item Shows the table
    \item Shows the table
    \item No red vertices
  \end{itemize}

\end{proof}

\begin{figure}[h]\centering
  \includegraphics[width=50pt]{images/cactus-reductions/p1-1.png}
  \caption[Reduction~\ref{rdc:p1-1}]{%
    }%
    Reduction \ref{rdc:p1-1}
    \label{fig:p1-1}
\end{figure}
\begin{restatable}{reduction}{reduction-p1}
  \label{rdc:p1-1}
  Contract the subgraph $P$ into vertex $0$ and remove 1 guards.
\end{restatable}

\begin{lemma}
  Reduction \ref{rdc:p1-1} is correct.
\end{lemma}
\begin{proof}

  \lowerbound

  Follows from Lemma \ref{lem:lb-seq} with $s = (3)$ and Lemma \ref{lem:contract-subgraph}.

  \upperbound


%5 - 1010: 5 6 8 11 
%6 - 0110: 5 6 8 11 
%8 - 0001: 5 6 8 11 
%11 - 1101: 5 6 8 11 

  \begin{itemize}

    \item Defending strategy:
  \begin{tabular}{|c|c|c|}
    \hline
    Name of state & Neighborhood of $S$ & Vertices of $S$\\
    \hline
    a & (0) & (2)\\
    \hline
    b & (1) & (2)\\
    \hline
    c & () & (3)\\
    \hline
    d & (0,1) & (3)\\
    \hline
  \end{tabular}

\item Every non-red vertex can be evicted in this strategy.

\item 

\item $\{0, 2\}$ and $\{1, 2\}$ are green by induction, the reduced edge is also green.

  \end{itemize}

\end{proof}

Application of reductions:
First pick a leaf biconnected component and check which of the following holds for it:
\begin{itemize}
  \item If there are two red vertices next to each other, do Reduction \ref{rdc:star2}
  \item If there is an induced $P_2$ on a cycle, use reduction \ref{rdc:p2}
  \item If there is a leaf connected to the cycle:
  \item If there is a vertex $v$ connected to a single leaf $l$:
    \begin{itemize}
      \item If $v$ has degree 2, then tree reduction
      \item If $v$ has degree 3, then it is on a cycle (TODO: show this)
        \begin{itemize}
          \item If both neighbors of $v$ are white, then Reduction \ref{rdc:p1-1}
          \item Otherwise perform
        \end{itemize}
    \end{itemize}
\end{itemize}

